The Effects of Dwarf Galaxies on the Orbital Evolution of Galactic Globular Clusters

We investigate the effect that dwarf galaxies have on the orbits, tidal histories, and assumed formation environment of Milky Way globular clusters. We determine the orbits of the Milky Way's 150 globular clusters in a gravitational potential both with and without dwarf galaxies. We find that the presence of a small number of satellite galaxies can affect the orbits of many of the globular clusters. Over 12 Gyr, we find that the semi-major axis and orbital eccentricity of individual clusters fluctuate with dispersions on the order of $\sim 10\%$ and $\sim 4\%$, respectively. Outer clusters are more strongly affected by dwarf galaxies than inner clusters, with their semi-major axis and orbital eccentricities fluctuating by more than $\sim 15\%$ and $\sim 5\%$, respectively. Using detailed $N$-body simulations of select clusters, we find that altering their orbital histories can lead to different mass loss rates and structural evolution. Furthermore, we caution against using kinematics alone to identify whether a Galactic cluster formed in-situ or was accreted during a past merger event as these values are no longer conserved. The presence of dwarf galaxies causes the orbital energies and actions of individual clusters to evolve over time, spanning a wider range than that coming from random uncertainties in a cluster's proper motions and radial velocity.

==> The Effect of Dwarf Galaxies on the Orbital Evolution of Globular Clusters/notes.tex <==
%% Define notes using todonotes package

\usepackage{xparse}
\usepackage{ifthen}

\makeatletter
% Increase margins for margin comments
\ifthenelse{\@todonotes@enable=1 \AND \@todonotes@inline=0}{
\paperwidth=\dimexpr\paperwidth + 6cm\relax
%\textwidth=\dimexpr \textwidth - 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@enable=1}
  {\usepackage[textwidth=\dimexpr\evensidemargin + 2.25cm]{todonotes}}
  {\usepackage[disable]{todonotes}}

% Colors for comment boxes
\definecolor{gold}{RGB}{255,215,0}
\definecolor{salmon}{rgb}{0.95,0.5,0.25}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{darkblue}{rgb}{0.0, 0., 0.7}
\definecolor{vlightblue}{rgb}{0.68,0.84,0.9}
\definecolor{purple}{rgb}{0.7, 0., 0.7}
\definecolor{lavender}{rgb}{0.9, 0.9, 0.98}

\newcommand{\@todonotes@loaded}{0}
\@ifpackageloaded{todonotes}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
% Deal with inline: hack
\ifthenelse{\@todonotes@inline=0}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
\@ifpackagewith{todonotes}{disable}
  {\renewcommand{\@todonotes@loaded}{0}}
  {}

% Increase margins for margin comments
%\ifthenelse{\@todonotes@loaded=1}{
%\textwidth=\dimexpr \textwidth - 6cm\relax
%\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
%\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
%\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@inline=1}{
\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[inline,backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
{\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
\makeatother

==> notes.tex <==
%% Define notes using todonotes package

\usepackage{xparse}
\usepackage{ifthen}

\makeatletter
% Increase margins for margin comments
\ifthenelse{\@todonotes@enable=1 \AND \@todonotes@inline=0}{
\paperwidth=\dimexpr\paperwidth + 6cm\relax
%\textwidth=\dimexpr \textwidth - 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@enable=1}
  {\usepackage[textwidth=\dimexpr\evensidemargin + 2.25cm]{todonotes}}
  {\usepackage[disable]{todonotes}}

% Colors for comment boxes
\definecolor{gold}{RGB}{255,215,0}
\definecolor{salmon}{rgb}{0.95,0.5,0.25}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{darkblue}{rgb}{0.0, 0., 0.7}
\definecolor{vlightblue}{rgb}{0.68,0.84,0.9}
\definecolor{purple}{rgb}{0.7, 0., 0.7}
\definecolor{lavender}{rgb}{0.9, 0.9, 0.98}

\newcommand{\@todonotes@loaded}{0}
\@ifpackageloaded{todonotes}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
% Deal with inline: hack
\ifthenelse{\@todonotes@inline=0}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
\@ifpackagewith{todonotes}{disable}
  {\renewcommand{\@todonotes@loaded}{0}}
  {}

% Increase margins for margin comments
%\ifthenelse{\@todonotes@loaded=1}{
%\textwidth=\dimexpr \textwidth - 6cm\relax
%\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
%\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
%\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@inline=1}{
\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[inline,backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
{\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
\makeatother
